Knowledge Distillation Layer that Lets the Student Decide

Typical technique in knowledge distillation (KD) is regularizing the learning of a limited capacity model (student) by pushing its responses to match a powerful model's (teacher). Albeit useful especially in the penultimate layer and beyond, its action on student's feature transform is rather implicit, limiting its practice in the intermediate layers. To explicitly embed the teacher's knowledge in feature transform, we propose a learnable KD layer for the student which improves KD with two distinct abilities: i) learning how to leverage the teacher's knowledge, enabling to discard nuisance information, and ii) feeding forward the transferred knowledge deeper. Thus, the student enjoys the teacher's knowledge during the inference besides training. Formally, we repurpose 1x1-BN-ReLU-1x1 convolution block to assign a semantic vector to each local region according to the template (supervised by the teacher) that the corresponding region of the student matches. To facilitate template learning in the intermediate layers, we propose a novel form of supervision based on the teacher's decisions. Through rigorous experimentation, we demonstrate the effectiveness of our approach on 3 popular classification benchmarks. Code is available at: https://github.com/adagorgun/letKD-framework

==> figures/fig_int_knowledge.tex <==

\begin{figure*}[!ht]
      \centering
      \centerline{\includegraphics[width=0.81\linewidth]{figures/fig_int_knowledge.png}}
    %  \vspace{2.0cm}
  \caption{Sample images with the teacher sub-class annotations marking the center of each spatial location.}
	\label{fig:int_knowledge}
  \end{figure*}

==> figures/fig_subclass_number.tex <==
% Below is an example of how to insert images. Delete the ``\vspace'' line,
% uncomment the preceding line ``\centerline...'' and replace ``imageX.ps''
% with a suitable PostScript file name.
% -------------------------------------------------------------------------
% \begin{wrapfigure}[10]{l}[-5pt]{0.47\linewidth}
% %\vspace{-.3\intextsep}
% %\begin{minipage}{.49\linewidth}
% %\begin{figure}[!ht]
%   %\centering
%   \centerline{\includegraphics[width=1.0\linewidth,keepaspectratio]{figures/subclass_number.png}}
%   %\smallskip
%   %\centerline{(b)}
%   %\end{figure}
% %\end{minipage}
% \caption{Effect of $K_{inter}$}
% \label{fig:subclass_number}
% \end{wrapfigure}

% \begin{wrapfigure}[13]{r}[-5pt]{0.485\linewidth} % 15
% \vspace{-3.2\intextsep} %\vspace{-2.5\intextsep}
%   %\centering
%   \centerline{\includegraphics[width=\linewidth]{figures/subclass_number.PNG}}
%   \caption{Effect of $K_{inter}$}
% 	\label{fig:subclass_number}
% \end{wrapfigure}

\begin{wrapfigure}[8]{r}[-2pt]{0.295\linewidth}
\vspace{-1.6\intextsep}
%\begin{minipage}{.49\linewidth}
%\begin{figure}[!ht]
  %\centering
  \centerline{\includegraphics[width=1.0\linewidth]{figures/subclass_number.png}}
  %\smallskip
  %\centerline{(b)}
  %\end{figure}
%\end{minipage}
\caption{Effect of $K_{inter}$}
\label{fig:subclass_number}
\end{wrapfigure}



% \begin{wrapfigure}[10]{l}[-5pt]{0.37\linewidth}
% \vspace{0\intextsep}
% %\begin{minipage}{.49\linewidth}
% %\begin{figure}[!ht]
%   %\centering
%   \centerline{\includegraphics[width=1.0\linewidth,keepaspectratio]{figures/subclass_number.png}}
%   %\smallskip
%   %\centerline{(b)}
%   %\end{figure}
% %\end{minipage}
% \caption{Effect of $K_{inter}$}
% \label{fig:subclass_number}
% \end{wrapfigure}

==> figures/table_CI.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[ht]%{r}[-5pt]{\linewidth}
    \vspace{-.75\intextsep}
    \centering
    \caption{Mean top-1 acc. with 95\% CI over 5 runs.}
    \label{tab:CI}
    \vspace{-.5\intextsep}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{ccccccccccc}
        \toprule 
        Dataset $\rightarrow$ & \multicolumn{6}{c}{\textbf{CIFAR-100}} & & \multicolumn{3}{c}{\textbf{Tiny-ImageNet}} \\ \cmidrule{2-7} \cmidrule{9-11}
        Setting $\rightarrow$ & \multicolumn{10}{c}{\textbf{Homogeneous Distillation}} \\ \midrule
        Teacher & WRN-40-2 & WRN-40-2 & RN56 & RN110 & RN110 & RN32x4 & & WRN-40-2 & WRN-40-2 & RN56 
        \\  
        Student & WRN-16-2 & WRN-40-1 & RN20 & RN20  & RN32  & RN8x4 & & WRN-16-2 & WRN-40-1 & RN20 
        \\ \midrule
        TDD & 75.01 & 74.04 & 71.53 & - & - & - & & 59.22 & 58.42 & 54.45 \\
        QUEST & 76.10 & 74.58 & 71.84 & 71.89 & 74.08 & 75.88 & & 59.86 & 59.13 & 54.53\\
        \midrule
        \textbf{letKD-1} & $\underset{\scriptsize{\mp0.15}}{76.29}$ & $\underset{\scriptsize{\mp0.09}}{75.01}$ & $\underset{\scriptsize{\mp0.24}}{72.44}$ & $\underset{\scriptsize{\mp0.31}}{72.68}$ & $\underset{\scriptsize{\mp0.14}}{74.40}$ & $\underset{\scriptsize{\mp0.06}}{76.70}$ & & $\underset{\scriptsize{\mp0.36}}{61.42}$  & $\underset{\scriptsize{\mp0.50}}{59.75}$ & $\underset{\scriptsize{\mp0.33}}{55.54}$ \\
        \textbf{letKD-2} & $\underset{\scriptsize{\mp0.22}}{76.56}$ & $\underset{\scriptsize{\mp0.13}}{75.19}$ & $\underset{\scriptsize{\mp0.16}}{73.27}$ & $\underset{\scriptsize{\mp0.14}}{73.38}$ & $\underset{\scriptsize{\mp0.20}}{74.62}$ & $\underset{\scriptsize{\mp0.18}}{77.09}$ & & $\underset{\scriptsize{\mp0.17}}{62.21}$ & $\underset{\scriptsize{\mp0.27}}{60.59}$ & $\underset{\scriptsize{\mp0.46}}{57.35}$ \\
        \midrule
        Setting $\rightarrow$ & \multicolumn{10}{c}{\textbf{Heterogeneous Distillation}} \\ \midrule
        {\begin{tabular}{c}
        Teacher \\
        Student \end{tabular}} &\multicolumn{6}{c}{\begin{tabular}{ccccccc}
        WRN-40-2 & & RN32x4 & & RN32x4 & & RN50 \\ SNV1 & & SNV1 & & SNV2 & & MNV2\end{tabular}} & 
        & 
        \multicolumn{3}{c}{\begin{tabular}{ccc} WRN-40-2 & & RN50 \\ SNV1 & & MNV2\end{tabular}} \\ \midrule
        {\begin{tabular}{c}
        TDD \\
        QUEST \end{tabular}} &\multicolumn{6}{c}{\begin{tabular}{ccccccc}
        75.60 & & - & & - & & 68.37 \\ 76.75 & & 76.28 & & 77.09 & & 69.81\end{tabular}} & 
        & 
        \multicolumn{3}{c}{\begin{tabular}{ccc} 65.27 & & 59.09 \\ 65.23 & & 59.81\end{tabular}} \\ \midrule
        {\begin{tabular}{c}
        \textbf{letKD-1} \\
        \textbf{letKD-2} \end{tabular}} &\multicolumn{6}{c}{\begin{tabular}{cccc}
        $\underset{\scriptsize{\mp0.16}}{76.93}$ & $\underset{\scriptsize{\mp0.24}}{76.65}$ & $\underset{\scriptsize{\mp0.17}}{77.75}$ & $\underset{\scriptsize{\mp0.18}}{69.97}$ \\ $\underset{\scriptsize{\mp0.12}}{77.08}$ & $\underset{\scriptsize{\mp0.12}}{77.30}$ & $\underset{\scriptsize{\mp0.06}}{77.95}$ & $\underset{\scriptsize{\mp0.23}}{70.39}$\end{tabular}} & 
        & 
        \multicolumn{3}{c}{\begin{tabular}{cc} $\underset{\scriptsize{\mp0.42}}{65.70}$ & $\underset{\scriptsize{\mp0.17}}{60.69}$ \\ $\underset{\scriptsize{\mp0.50}}{66.15}$ & $\underset{\scriptsize{\mp0.46}}{61.15}$\end{tabular}} \\ \bottomrule
        \end{tabular}%
     }
\end{table}

==> figures/table_CIFAR100_crossmodel.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\begin{table*}[ht]%[13]{r}[-5pt]{0.6\linewidth}
    %\vspace{-.9\intextsep}
	\centering
	\caption{\textbf{Evaluation on CIFAR-100.} Top-1 accuracy of heterogeneous distillation on CIFAR-100. The results for other methods are taken from \cite{jain2019quest} and \cite{Zhao_2022_CVPR}. All results are the average over 5 trials. \textbf{Bold}: best in its category.}
	\label{tab:cifar100_cross}
	\begin{tabular}{ccccc}
		\toprule 
		Teacher & WRN-40-2     & ResNet32x4   & ResNet32x4   & ResNet50   \\  
		Student & ShuffleNetV1 & ShuffleNetV1 & ShuffleNetV2 & MobileNetV2\\ \midrule
		Teacher & 75.61        & 79.42        & 79.42        & 79.34      \\
		Student & 70.50        & 70.50        & 71.82        & 64.60      \\ \midrule
        KD & 74.83 & 74.07 & 74.45 & 67.35 \\ 
        FitNet & 73.73 & 73.59 & 73.54 & 63.16 \\
        AT & 73.32 & 71.73 & 72.73 & 58.58 \\
        AB & 73.34 & 73.55 & 74.31 & 67.20 \\ 
        SP & 74.52 & 73.48 & 74.56 & 68.08 \\
        VID & 73.61 & 73.38 & 73.40 & 67.57 \\
        CRD & 76.05 & 75.11 & 75.65 & 69.11 \\
        CRD+KD & 76.27 & 75.12 & 76.05 & 69.54 \\
        DKD & 76.70 & 76.45 & 77.07 & 70.35 \\
        SimKD & 76.95 & 77.18 & 77.78 & 68.91 \\
        TDD & 75.60 & - & - & 68.37 \\
        TDD+CRD & 76.34 & - & - & 69.22 \\
        QUEST & 76.75 & 76.28 & 77.09 & 69.81 \\
        \midrule
        \textbf{letKD-1} & 76.93 & 76.65 & 77.75 & 69.97 \\
        \textbf{letKD-2} & \textbf{77.08} & \textbf{77.30} & \textbf{77.95} & \textbf{70.39} \\
		\bottomrule
	\end{tabular}%
\end{table*}


==> figures/table_CIFAR100_crossmodel_ref.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\begin{table*}[ht]%[13]{r}[-5pt]{0.6\linewidth}
    %\vspace{-.9\intextsep}
	\centering
	\caption{Evaluation on image recognition task. Bold: best in its category. $C:$ the number of classes.}
	\label{tab:alldata}
	\begin{tabular}{ccccc}
		\toprule 
		Teacher & WRN-40-2     & ResNet32x4   & ResNet32x4   & ResNet50   \\  
		Student & ShuffleNetV1 & ShuffleNetV1 & ShuffleNetV2 & MobileNetv2\\ \midrule
		Teacher & 75.61        & 79.42        & 79.42        & 79.34      \\
		Student & 70.50        & 70.50        & 71.82        & 64.60      \\ \midrule
        KD \cite{Hinton2015} & 74.83 & 74.07 & 74.45 & 67.35 \\ 
        FitNet \cite{FitNet} & 73.73 & 73.59 & 73.54 & 63.16 \\
        AT \cite{zagoruyko2017paying} & 73.32 & 71.73 & 72.73 & 67.20 \\
        AB \cite{heo2019AB} & 73.34 & 73.55 & 74.31 & 67.20 \\ 
        SP \cite{Tung_2019_ICCV} & 74.52 & 73.48 & 74.56 & 68.08 \\
        VID \cite{Ahn_2019_CVPR} & 73.61 & 73.38 & 73.40 & 67.57 \\
        CRD \cite{tian2019crd} & 76.05 & 75.11 & 75.65 & 69.11 \\
        CRD+KD \cite{tian2019crd} & 76.27 & 75.12 & 76.05 & 69.54 \\
        DKD \cite{Zhao_2022_CVPR} & 76.70 & 76.45 & 77.07 & 70.35 \\
        SimKD \cite{Chen_2022_CVPR} & 76.95 & 77.18 & 77.78 & 68.91 \\
        TDD \cite{Song_2021_CVPR} & 75.60 & - & - & 68.37 \\
        TDD+CRD \cite{Song_2021_CVPR} & 76.34 & - & - & 69.22 \\
        QUEST \cite{jain2019quest} & 76.75 & 76.28 & 77.09 & 69.81 \\
        \midrule
        \textbf{letKD-1} & 76.93 & 76.65 & 77.75 & 69.97 \\
        \textbf{letKD-2} & \textbf{77.08} & \textbf{77.30} & \textbf{77.95} & \textbf{70.39} \\
		\bottomrule
	\end{tabular}%
\end{table*}


==> figures/table_CIFAR100_homogeneous.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\begin{table*}[ht]%[13]{r}[-5pt]{0.6\linewidth}
    %\vspace{-.9\intextsep}
	\centering
	\caption{\textbf{Evaluation on CIFAR-100.} Top-1 accuracy of homogeneous distillation on CIFAR-100. The results for other methods are taken from \cite{jain2019quest} and \cite{Zhao_2022_CVPR}. All results are the average over 5 trials. \textbf{Bold}: best in its category.}
	\label{tab:cifar100_homogeneous}
	\begin{tabular}{ccccccc}
		\toprule 
		Teacher & WRN-40-2 & WRN-40-2 & ResNet56 & ResNet110 & ResNet110 & ResNet32x4\\  
		Student & WRN-16-2 & WRN-40-1 & ResNet20 & ResNet20  & ResNet32  & ResNet8x4 \\ \midrule
		Teacher & 75.61    & 75.61    & 72.34    & 74.31     & 74.31     & 79.42     \\
		Student & 73.26    & 71.98    & 69.06    & 69.06     & 71.14     & 72.50     \\ \midrule
        KD & 74.92 & 73.54 & 70.66 & 70.67 & 73.08 & 73.33 \\
        FitNet & 73.58 & 72.24 & 69.21 & 68.99 & 71.06 & 73.50 \\
        AT & 74.08 & 72.77 & 70.55 & 70.22 & 72.31 & 73.44 \\
        AB & 72.50 & 72.38 & 69.47 & 69.53 & 70.98 & 73.17 \\
        FSP & 72.91 & - & 69.95 & 70.11 & 71.89 & 72.62 \\
        SP & 73.83 & 72.43 & 69.67 & 70.04 & 72.69 & 72.94 \\
        VID & 74.11 & 73.30 & 70.38 & 70.16 & 72.61 & 73.09 \\
        CRD & 75.48 & 74.14 & 71.16 & 71.46 & 73.48 & 75.51 \\
        CRD+KD & 75.64 & 74.38 & 71.63 & 71.56 & 73.75 & 75.46 \\
        DKD & 76.24 & 74.81 & 71.97 & - & 74.11 & 76.32 \\
        SimKD & 76.06 & 74.92 & 68.95 & 69.35 & 72.15 & \textbf{78.08} \\
        TDD & 75.01 & 74.04 & 71.53 & - & - & - \\
        TDD+CRD & 75.71 & 74.35 & 71.88 & - & - & - \\
        QUEST & 76.10 & 74.58 & 71.84 & 71.89 & 74.08 & 75.88 \\
        \midrule
        \textbf{letKD-1} & 76.29 & 75.01 & 72.44 & 72.68 & 74.40 & 76.70 \\
        \textbf{letKD-2} & \textbf{76.56} & \textbf{75.19} & \textbf{73.27} & \textbf{73.39} & \textbf{74.62} & 77.09 \\
		\bottomrule
	\end{tabular}%
\end{table*}


==> figures/table_CIFAR100_homogeneous_ref.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\begin{table*}[ht]%[13]{r}[-5pt]{0.6\linewidth}
    %\vspace{-.9\intextsep}
	\centering
	\caption{Evaluation on image recognition task. Bold: best in its category. $C:$ the number of classes.}
	\label{tab:alldata}
	\begin{tabular}{ccccccc}
		\toprule 
		Teacher & WRN-40-2 & WRN-40-2 & ResNet56 & ResNet110 & ResNet110 & ResNet32x4\\  
		Student & WRN-16-2 & WRN-40-1 & ResNet20 & ResNet20  & ResNet32  & ResNet8x4 \\ \midrule
		Teacher & 75.61    & 75.61    & 72.34    & 74.31     & 74.31     & 79.42     \\
		Student & 73.26    & 71.98    & 69.06    & 69.06     & 71.14     & 72.50     \\ \midrule
        KD \cite{Hinton2015} & 74.92 & 73.54 & 70.66 & 70.67 & 73.08 & 73.33 \\
        FitNet \cite{FitNet} & 73.58 & 72.24 & 69.21 & 68.99 & 71.06 & 73.50 \\
        AT \cite{zagoruyko2017paying} & 74.08 & 72.77 & 70.55 & 70.22 & 72.31 & 73.44 \\
        AB \cite{heo2019AB} & 72.50 & 72.38 & 69.47 & 69.53 & 70.98 & 73.17 \\
        FSP \cite{yim2017FSP} & 72.91 & - & 69.95 & 70.11 & 71.89 & 72.62 \\
        SP \cite{Tung_2019_ICCV} & 73.83 & 72.43 & 69.67 & 70.04 & 72.69 & 72.94 \\
        VID \cite{Ahn_2019_CVPR} & 74.11 & 73.30 & 70.38 & 70.16 & 72.61 & 73.09 \\
        CRD \cite{tian2019crd} & 75.48 & 74.14 & 71.16 & 71.46 & 73.48 & 75.51 \\
        CRD+KD \cite{tian2019crd} & 75.64 & 74.38 & 71.63 & 71.56 & 73.75 & 75.46 \\
        DKD \cite{Zhao_2022_CVPR} & 76.24 & 74.81 & 71.97 & - & 74.11 & 76.32 \\
        SimKD \cite{Chen_2022_CVPR} & 76.06 & 74.92 & 68.95 & 69.35 & 72.15 & \textbf{78.08} \\
        TDD \cite{Song_2021_CVPR} & 75.01 & 74.04 & 71.53 & - & - & - \\
        TDD+CRD \cite{Song_2021_CVPR} & 75.71 & 74.35 & 71.88 & - & - & - \\
        QUEST \cite{jain2019quest} & 76.10 & 74.58 & 71.84 & 71.89 & 74.08 & 75.88 \\
        \midrule
        \textbf{letKD-1} & 76.29 & 75.01 & 72.44 & 72.68 & 74.40 & 76.70 \\
        \textbf{letKD-2} & \textbf{76.56} & \textbf{75.19} & \textbf{73.27} & \textbf{73.39} & \textbf{74.62} & 77.09 \\
		\bottomrule
	\end{tabular}%
\end{table*}


==> figures/table_CIFAR100_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\begin{table*}[ht]%[13]{r}[-5pt]{0.6\linewidth}
    %\vspace{-.9\intextsep}
	\centering
	\caption{Average top-1 accuracies on CIFAR-100 over 5 trials. \textbf{Bold}: best in its category.}
	\label{tab:cifar100}
	\resizebox{\linewidth}{!}{%
    	\begin{tabular}{cccccccccccc}
    		\toprule 
    		Archs. $\rightarrow$ & \multicolumn{6}{c}{\textbf{Homogeneous}} & & \multicolumn{4}{c}{\textbf{Heterogeneous}} \\ \cmidrule{2-7} \cmidrule{9-12} 
    		Teacher & WRN-40-2 & WRN-40-2 & RN56 & RN110 & RN110 & RN32x4 & & WRN-40-2 & RN32x4 & RN32x4 & RN50\\  
    		Student & WRN-16-2 & WRN-40-1 & RN20 & RN20  & RN32  & RN8x4 & & SNV1 & SNV1 & SNV2 & MNV2\\ \midrule
    		\multirow{2}{*}{Methods $\downarrow$} & 75.61 & 75.61 & 72.34 & 74.31 & 74.31 & 79.42 & & 75.61 & 79.42 & 79.42 & 79.34 \\
    		 & 73.26 & 71.98 & 69.06 & 69.06 & 71.14 & 72.50 & & 70.50 & 70.50 & 71.82 & 64.60 \\ \midrule
            KD & 74.92 & 73.54 & 70.66 & 70.67 & 73.08 & 73.33 & & 74.83 & 74.07 & 74.45 & 67.35\\
            FitNet & 73.58 & 72.24 & 69.21 & 68.99 & 71.06 & 73.50 & & 73.73 & 73.59 & 73.54 & 63.16 \\
            AT & 74.08 & 72.77 & 70.55 & 70.22 & 72.31 & 73.44 & & 73.32 & 71.73 & 72.73 & 58.58 \\
            AB & 72.50 & 72.38 & 69.47 & 69.53 & 70.98 & 73.17 & & 73.34 & 73.55 & 74.31 & 67.20 \\
            FSP & 72.91 & - & 69.95 & 70.11 & 71.89 & 72.62 & & - & - & - & - \\
            SP & 73.83 & 72.43 & 69.67 & 70.04 & 72.69 & 72.94 & & 74.52 & 73.48 & 74.56 & 68.08 \\
            VID & 74.11 & 73.30 & 70.38 & 70.16 & 72.61 & 73.09 & & 73.61 & 73.38 & 73.40 & 67.57 \\
            CRD & 75.48 & 74.14 & 71.16 & 71.46 & 73.48 & 75.51 & & 76.05 & 75.11 & 75.65 & 69.11 \\
            $\underset{\text{+KD}}{\text{CRD}}$ & 75.64 & 74.38 & 71.63 & 71.56 & 73.75 & 75.46 & & 76.27 & 75.12 & 76.05 & 69.54\\
            DKD & 76.24 & 74.81 & 71.97 & - & 74.11 & 76.32 & & 76.70 & 76.45 & 77.07 & 70.35 \\
            SimKD & 76.06 & 74.92 & 68.95 & 69.35 & 72.15 & \textbf{78.08} & & 76.95 & 77.18 & 77.78 & 68.91 \\
            TDD & 75.01 & 74.04 & 71.53 & - & - & - & & 75.60 & - & - & 68.37 \\
            $\underset{\text{+CRD}}{\text{TDD}}$ & 75.71 & 74.35 & 71.88 & - & - & - & & 76.34 & - & - & 69.22 \\
            QUEST & 76.10 & 74.58 & 71.84 & 71.89 & 74.08 & 75.88 & & 76.75 & 76.28 & 77.09 & 69.81 \\
            \midrule
            \textbf{letKD-1} & 76.29 & 75.01 & 72.44 & 72.68 & 74.40 & 76.70 & & 76.93 & 76.65 & 77.75 & 69.97 \\
            \textbf{letKD-2} & \textbf{76.56} & \textbf{75.19} & \textbf{73.27} & \textbf{73.39} & \textbf{74.62} & 77.09 & & \textbf{77.08} & \textbf{77.30} & \textbf{77.95} & \textbf{70.39} \\
    		\bottomrule
    	\end{tabular}%
    }
\end{table*}


==> figures/table_CI_CIFAR100.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\begin{wraptable}[3]{r}[-5pt]{\linewidth}
    %\vspace{-.9\intextsep}
	\centering
	\caption{Top-1 acc. averaged over 5 trials on CIFAR100 with 95\% CI. \textbf{Bold}: best in its category.}
	\label{tab:cifar100_CI}
        \resizebox{\linewidth}{!}{%
    	\begin{tabular}{cccccccccccc}
    		\toprule 
    		Archs. $\rightarrow$ & \multicolumn{6}{c}{\textbf{Homogeneous}} & & \multicolumn{4}{c}{\textbf{Heterogeneous}} \\ \cmidrule{2-7} \cmidrule{9-12}
    		Teacher & WRN-40-2 & WRN-40-2 & RN56 & RN110 & RN110 & RN32x4 & & WRN-40-2 & RN32x4 & RN32x4 & RN50 \\  
    		Student & WRN-16-2 & WRN-40-1 & RN20 & RN20  & RN32  & RN8x4 & & SNV1 & SNV1 & SNV2 & MNV2 \\ \midrule
    		\multirow{2}{*}{Methods $\downarrow$} & 75.61 & 75.61 & 72.34 & 74.31 & 74.31 & 79.42 & & 75.61 & 79.42 & 79.42 & 79.34 \\
    		 & 73.26 & 71.98 & 69.06 & 69.06 & 71.14 & 72.50 & & 70.50 & 70.50 & 71.82 & 64.60 \\ \midrule
            TDD & 75.01 & 74.04 & 71.53 & - & - & - & & 75.60 & - & - & 68.37\\
            QUEST & 76.10 & 74.58 & 71.84 & 71.89 & 74.08 & 75.88 & & 76.75 & 76.28 & 77.09 & 69.81\\
            \midrule
            \textbf{letKD-1} & 76.29 {\footnotesize $\pm$0.15} & 75.01 {\footnotesize $\pm$0.09} & 72.44 {\footnotesize $\pm$0.24}  & 72.68 {\footnotesize $\pm$0.31} & 74.40 {\footnotesize $\pm$0.14} & 76.70 {\footnotesize $\pm$0.06} & & 76.93 {\footnotesize $\pm$0.16} & 76.65 {\footnotesize $\pm$0.24} & 77.75 {\footnotesize $\pm$0.17} & 69.97 {\footnotesize $\pm$0.18} \\
            \textbf{letKD-2} & \textbf{76.56 {\footnotesize $\pm$0.22}} & \textbf{75.19 {\footnotesize $\pm$0.13}} & \textbf{73.27 {\footnotesize $\pm$0.16}} & \textbf{73.38 {\footnotesize $\pm$0.14}} & \textbf{74.62 {\footnotesize $\pm$0.20}} & \textbf{77.09 {\footnotesize $\pm$0.18}} & & \textbf{77.08 {\footnotesize $\pm$0.12}} & \textbf{77.30 {\footnotesize $\pm$0.12}} & \textbf{77.95 {\footnotesize $\pm$0.06}} & \textbf{70.39 {\footnotesize $\pm$0.23}} \\
    		\bottomrule
    	\end{tabular}%
     }
\end{wraptable}

==> figures/table_CI_Tiny.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\begin{wraptable}[3]{r}[-5pt]{\linewidth}
% \begin{wraptable}[15]{r}[-5pt]{0.5\linewidth}
    % \vspace{-.9\intextsep}
    % \vspace{-10}
	\centering
	\caption{Top-1 acc. averaged over 3 trials on Tiny-ImageNet with 95\% CI. \textbf{Bold}: best in its category.}
	\label{tab:tinyimagenet_CI}
	\resizebox{.5\linewidth}{!}{%
	\begin{tabular}{ccccccc}
		\toprule 
		Archs. $\rightarrow$ & \multicolumn{3}{c}{\textbf{Homogeneous}} & & \multicolumn{2}{c}{\textbf{Heterogeneous}} \\ \cmidrule{2-4} \cmidrule{6-7}
		Teacher & WRN-40-2 & WRN-40-2 & RN56 & & WRN-40-2 & RN50 \\  
		Student & WRN-16-2 & WRN-40-1 & RN20 & & SNV1  & MNV2 \\ \midrule
		\multirow{2}{*}{Methods $\downarrow$} & 61.26 & 61.26 & 58.34 & & 61.26 & 68.97 \\
		& 57.17 & 56.25 & 52.66 & & 60.52 & 58.35 \\ \midrule
        TDD & 59.22 & 58.42 & 54.45 & & 65.27 & 59.09 \\
        QUEST & 59.86 & 59.13 & 54.53 & & 65.23 & 59.81 \\
        \midrule
        \textbf{letKD-1} & 61.42 {\footnotesize $\pm$0.36} & 59.75 {\footnotesize $\pm$0.50} & 55.54 {\footnotesize $\pm$0.33} & & 65.70 {\footnotesize $\pm$0.42} & 60.69 {\footnotesize $\pm$0.17}\\
        \textbf{letKD-2} & \textbf{62.21 {\footnotesize $\pm$0.17}} & \textbf{60.59 {\footnotesize $\pm$0.27}} & \textbf{57.35 {\footnotesize $\pm$0.46}} & & \textbf{66.15 {\footnotesize $\pm$0.50}} & \textbf{61.15 {\footnotesize $\pm$0.46}} \\
		\bottomrule
	\end{tabular}%
	}
\end{wraptable}


==> figures/table_CI_class_underset.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\begin{table}[h]
    % \vspace{-.8\intextsep}
    \centering
    \caption{Mean top-1 acc. with 95\% CI over multiple runs.}
    \vspace{-.6\intextsep}
    \label{tab:CI_class_underset}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{cccccccccccc}
    \toprule        
    Dataset $\rightarrow$ & \multicolumn{11}{c}{\textbf{CIFAR-100}}\\ \midrule
    Archs. $\rightarrow$ & \multicolumn{6}{c}{\textbf{Homogeneous}} & & \multicolumn{4}{c}{\textbf{Heterogeneous}} \\ \cmidrule{2-7} \cmidrule{9-12}
    Teacher & WRN-40-2 & WRN-40-2 & RN56 & RN110 & RN110 & RN32x4 & & WRN-40-2 & RN32x4 & RN32x4 & RN50 \\  
    Student & WRN-16-2 & WRN-40-1 & RN20 & RN20  & RN32  & RN8x4 & & SNV1 & SNV1 & SNV2 & MNV2 \\ \midrule
    TDD & 75.01 & 74.04 & 71.53 & - & - & - & & 75.60 & - & - & 68.37\\
    QUEST & 76.10 & 74.58 & 71.84 & 71.89 & 74.08 & 75.88 & & 76.75 & 76.28 & 77.09 & 69.81\\
    \midrule
    \textbf{letKD-1} & 
    $\underset{\scriptsize{\mp0.15}}{76.29}$ & $\underset{\scriptsize{\mp0.09}}{75.01}$ & $\underset{\scriptsize{\mp0.24}}{72.44}$ & $\underset{\scriptsize{\mp0.31}}{72.68}$ & $\underset{\scriptsize{\mp0.14}}{74.40}$ & $\underset{\scriptsize{\mp0.06}}{76.70}$ & & $\underset{\scriptsize{\mp0.16}}{76.93}$ & $\underset{\scriptsize{\mp0.24}}{76.65}$ & $\underset{\scriptsize{\mp0.17}}{77.75}$ &
    $\underset{\scriptsize{\mp0.18}}{69.97}$
    \\
    \textbf{letKD-2} & 
    $\mathbf{\underset{\scriptsize{\mp0.22}}{76.56}}$ & $\mathbf{\underset{\scriptsize{\mp0.13}}{75.19}}$ & $\mathbf{\underset{\scriptsize{\mp0.16}}{73.27}}$ & $\mathbf{\underset{\scriptsize{\mp0.14}}{73.38}}$ & $\mathbf{\underset{\scriptsize{\mp0.20}}{74.62}}$ & $\mathbf{\underset{\scriptsize{\mp0.18}}{77.09}}$ & & $\mathbf{\underset{\scriptsize{\mp0.12}}{77.08}}$ & $\mathbf{\underset{\scriptsize{\mp0.12}}{77.30}}$ & $\mathbf{\underset{\scriptsize{\mp0.06}}{77.95}}$ &
    $\mathbf{\underset{\scriptsize{\mp0.23}}{70.39}}$ 
    \\
    \midrule
    Dataset $\rightarrow$ & \multicolumn{11}{c}{\textbf{Tiny-ImageNet}}\\ \midrule
    Archs. $\rightarrow$ & \multicolumn{6}{c}{\textbf{Homogeneous}} & & \multicolumn{4}{c}{\textbf{Heterogeneous}} \\ \cmidrule{2-7} \cmidrule{9-12}
    Teacher & \multicolumn{2}{c}{WRN-40-2} & \multicolumn{2}{c}{WRN-40-2} & \multicolumn{2}{c}{RN56} & & \multicolumn{2}{c}{WRN-40-2} & \multicolumn{2}{c}{RN50} \\  
    Student & \multicolumn{2}{c}{WRN-16-2} & \multicolumn{2}{c}{WRN-40-1} & \multicolumn{2}{c}{RN20} & & \multicolumn{2}{c}{SNV1}  & \multicolumn{2}{c}{MNV2} \\ \midrule
    TDD & \multicolumn{2}{c}{59.22} & \multicolumn{2}{c}{58.42} & \multicolumn{2}{c}{54.45} & & \multicolumn{2}{c}{65.27} & \multicolumn{2}{c}{59.09} \\
    QUEST & \multicolumn{2}{c}{59.86} & \multicolumn{2}{c}{59.13} & \multicolumn{2}{c}{54.53} & & \multicolumn{2}{c}{65.23} & \multicolumn{2}{c}{59.81} \\
    \midrule
    \textbf{letKD-1} & 
    \multicolumn{2}{c}{$\underset{\scriptsize{\mp0.36}}{61.42}$} & \multicolumn{2}{c}{$\underset{\scriptsize{\mp0.50}}{59.75}$} & \multicolumn{2}{c}{$\underset{\scriptsize{\mp0.33}}{55.54}$} & & 
    \multicolumn{2}{c}{$\underset{\scriptsize{\mp0.42}}{65.70}$} & \multicolumn{2}{c}{$\underset{\scriptsize{\mp0.17}}{60.69}$}
    \\
    \textbf{letKD-2} & 
    \multicolumn{2}{c}{$\mathbf{\underset{\scriptsize{\mp0.17}}{62.21}}$} & \multicolumn{2}{c}{$\mathbf{\underset{\scriptsize{\mp0.27}}{60.59}}$} & \multicolumn{2}{c}{$\mathbf{\underset{\scriptsize{\mp0.46}}{57.35}}$} & &
    \multicolumn{2}{c}{$\mathbf{\underset{\scriptsize{\mp0.50}}{66.15}}$} & \multicolumn{2}{c}{$\mathbf{\underset{\scriptsize{\mp0.46}}{61.15}}$}
    \\
    \bottomrule
    \end{tabular}%
     }
\end{table}

==> figures/table_CI_deneme.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[ht]%{r}[-5pt]{\linewidth}
    \vspace{-.8\intextsep}
    \centering
    \caption{Mean top-1 acc. with 95\% CI over 5 runs.}
    \label{tab:CI}
    \vspace{-.5\intextsep}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{ccccccccccc}
        \toprule 
        Dataset $\rightarrow$ & \multicolumn{6}{c}{\textbf{CIFAR-100}} & & \multicolumn{3}{c}{\textbf{Tiny-ImageNet}} \\ \cmidrule{2-7} \cmidrule{9-11}
        Setting $\rightarrow$ & \multicolumn{10}{c}{\textbf{Homogeneous Distillation}} \\ \midrule
        Teacher & WRN-40-2 & WRN-40-2 & RN56 & RN110 & RN110 & RN32x4 & & WRN-40-2 & WRN-40-2 & RN56 
        \\  
        Student & WRN-16-2 & WRN-40-1 & RN20 & RN20  & RN32  & RN8x4 & & WRN-16-2 & WRN-40-1 & RN20 
        \\ \midrule
        TDD & 75.01 & 74.04 & 71.53 & - & - & - & & 59.22 & 58.42 & 54.45 \\
        QUEST & 76.10 & 74.58 & 71.84 & 71.89 & 74.08 & 75.88 & & 59.86 & 59.13 & 54.53\\
        \midrule
        \textbf{letKD-1} & $\underset{\scriptsize{\mp0.15}}{76.29}$ & $\underset{\scriptsize{\mp0.09}}{75.01}$ & $\underset{\scriptsize{\mp0.24}}{72.44}$ & $\underset{\scriptsize{\mp0.31}}{72.68}$ & $\underset{\scriptsize{\mp0.14}}{74.40}$ & $\underset{\scriptsize{\mp0.06}}{76.70}$ & & $\underset{\scriptsize{\mp0.36}}{61.42}$  & $\underset{\scriptsize{\mp0.50}}{59.75}$ & $\underset{\scriptsize{\mp0.33}}{55.54}$ \\
        \textbf{letKD-2} & $\underset{\scriptsize{\mp0.22}}{76.56}$ & $\underset{\scriptsize{\mp0.13}}{75.19}$ & $\underset{\scriptsize{\mp0.16}}{73.27}$ & $\underset{\scriptsize{\mp0.14}}{73.38}$ & $\underset{\scriptsize{\mp0.20}}{74.62}$ & $\underset{\scriptsize{\mp0.18}}{77.09}$ & & $\underset{\scriptsize{\mp0.17}}{62.21}$ & $\underset{\scriptsize{\mp0.27}}{60.59}$ & $\underset{\scriptsize{\mp0.46}}{57.35}$ \\
        \midrule
        Setting $\rightarrow$ & \multicolumn{10}{c}{\textbf{Heterogeneous Distillation}} \\ \midrule
        {\begin{tabular}{c}
        Teacher \\
        Student \end{tabular}} &\multicolumn{6}{c}{\begin{tabular}{ccccccc}
        WRN-40-2 & & RN32x4 & & RN32x4 & & RN50 \\ SNV1 & & SNV1 & & SNV2 & & MNV2\end{tabular}} & 
        & 
        \multicolumn{3}{c}{\begin{tabular}{ccc} WRN-40-2 & & RN50 \\ SNV1 & & MNV2\end{tabular}} \\ \midrule
        {\begin{tabular}{c}
        TDD \\
        QUEST \end{tabular}} &\multicolumn{6}{c}{\begin{tabular}{cccccccc}
        75.60 & & & - & & - & & 68.37 \\ 76.75 & & 76.28 & & 77.09 & & 69.81\end{tabular}} & 
        & 
        \multicolumn{3}{c}{\begin{tabular}{ccc} 65.27 & & 59.09 \\ 65.23 & & 59.81\end{tabular}} \\ \midrule
        {\begin{tabular}{c}
        \textbf{letKD-1}  \\
        \textbf{letKD-2} \end{tabular}} &\multicolumn{6}{c}{\begin{tabular}{cccc}
        $\underset{\scriptsize{\mp0.16}}{76.93}$ & $\underset{\scriptsize{\mp0.24}}{76.65}$ & $\underset{\scriptsize{\mp0.17}}{77.75}$ & $\underset{\scriptsize{\mp0.18}}{69.97}$ \\ $\underset{\scriptsize{\mp0.12}}{77.08}$ & $\underset{\scriptsize{\mp0.12}}{77.30}$ & $\underset{\scriptsize{\mp0.06}}{77.95}$ & $\underset{\scriptsize{\mp0.23}}{70.39}$\end{tabular}} & 
        & 
        \multicolumn{3}{c}{\begin{tabular}{cc} $\underset{\scriptsize{\mp0.42}}{65.70}$ & $\underset{\scriptsize{\mp0.17}}{60.69}$ \\ $\underset{\scriptsize{\mp0.50}}{66.15}$ & $\underset{\scriptsize{\mp0.46}}{61.15}$\end{tabular}} \\ \bottomrule
        \end{tabular}%
     }
\end{table}

==> figures/table_CI_heterogeneous_CIFAR100.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\begin{wraptable}[3]{r}[-5pt]{\linewidth}
    %\vspace{-.9\intextsep}
	\centering
	\caption{Top-1 acc. averaged over 5 trials on CIFAR100 with 95\% CI for heterogeneous distillation. \textbf{Bold}: best in its category.}
	\label{tab:cifar100_CI_heterogeneous}
	\resizebox{.5\linewidth}{!}{%
    	\begin{tabular}{cccccc}
    		\toprule 
    		Archs. $\rightarrow$ & \multicolumn{4}{c}{\textbf{Heterogeneous}} \\ \cmidrule{2-5} 
    		Teacher & WRN-40-2 & RN32x4 & RN32x4 & RN50\\  
    		Student & SNV1 & SNV1 & SNV2 & MNV2\\ \midrule
    		\multirow{2}{*}{Methods $\downarrow$} & 75.61 & 79.42 & 79.42 & 79.34 \\
    		 & 70.50 & 70.50 & 71.82 & 64.60 \\ \midrule
            TDD & 75.60 & - & - & 68.37 \\
            QUEST & 76.75 & 76.28 & 77.09 & 69.81 \\
            \midrule
            \textbf{letKD-1} & 76.93 {\footnotesize $\pm$0.16} & 76.65 {\footnotesize $\pm$0.24} & 77.75 {\footnotesize $\pm$0.17} & 69.97 {\footnotesize $\pm$0.18} \\
            \textbf{letKD-2} & \textbf{77.08 {\footnotesize $\pm$0.12}} & \textbf{77.30 {\footnotesize $\pm$0.12}} & \textbf{77.95 {\footnotesize $\pm$0.06}} & \textbf{70.39 {\footnotesize $\pm$0.23}} \\
    		\bottomrule
    	\end{tabular}%
    }
\end{wraptable}


==> figures/table_CI_heterogeneous_Tiny.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\begin{wraptable}[3]{r}[-5pt]{\linewidth}
% \begin{wraptable}[15]{r}[-5pt]{0.5\linewidth}
    % \vspace{-.9\intextsep}
    % \vspace{-10}
	\centering
	\caption{Top-1 acc. averaged over 3 trials on Tiny-ImageNet with 95\% CI for heterogeneous distillation. \textbf{Bold}: best in its category.}
	\label{tab:tinyimagenet_CI_heterogeneous}
	\resizebox{.6\linewidth}{!}{%
	\begin{tabular}{cccc}
		\toprule 
		Archs. $\rightarrow$ & \multicolumn{2}{c}{\textbf{Heterogeneous}} \\ \cmidrule{2-3}
		Teacher & WRN-40-2 & RN50 \\  
		Student & SNV1  & MNV2 \\ \midrule
		\multirow{2}{*}{Methods $\downarrow$} & 61.26 & 68.97 \\
		& 60.52 & 58.35 \\ \midrule
        TDD & 65.27 & 59.09 \\
        QUEST & 65.23 & 59.81 \\
        \midrule
        \textbf{letKD-1} & 65.70 {\footnotesize $\pm$0.42} & 60.69 {\footnotesize $\pm$0.17} \\
        \textbf{letKD-2} & \textbf{66.15 {\footnotesize $\pm$0.50}} & \textbf{61.15 {\footnotesize $\pm$0.46}} \\
		\bottomrule
	\end{tabular}%
	}
\end{wraptable}


==> figures/table_CI_homogeneous_CIFAR100.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\begin{wraptable}[3]{r}[-5pt]{\linewidth}
    %\vspace{-.9\intextsep}
	\centering
	\caption{Top-1 acc. averaged over 5 trials on CIFAR100 with 95\% CI for homogeneous distillation. \textbf{Bold}: best in its category.}
	\label{tab:cifar100_CI_homogeneous}
        \resizebox{.5\linewidth}{!}{%
    	\begin{tabular}{ccccccc}
    		\toprule 
    		Archs. $\rightarrow$ & \multicolumn{6}{c}{\textbf{Homogeneous}} \\ \cmidrule{2-7}
    		Teacher & WRN-40-2 & WRN-40-2 & RN56 & RN110 & RN110 & RN32x4 \\  
    		Student & WRN-16-2 & WRN-40-1 & RN20 & RN20  & RN32  & RN8x4 \\ \midrule
    		\multirow{2}{*}{Methods $\downarrow$} & 75.61 & 75.61 & 72.34 & 74.31 & 74.31 & 79.42 \\
    		 & 73.26 & 71.98 & 69.06 & 69.06 & 71.14 & 72.50 \\ \midrule
            TDD & 75.01 & 74.04 & 71.53 & - & - & - \\
            QUEST & 76.10 & 74.58 & 71.84 & 71.89 & 74.08 & 75.88\\
            \midrule
            \textbf{letKD-1} & 76.29 {\footnotesize $\pm$0.15} & 75.01 {\footnotesize $\pm$0.09} & 72.44 {\footnotesize $\pm$0.24}  & 72.68 {\footnotesize $\pm$0.31} & 74.40 {\footnotesize $\pm$0.14} & 76.70 {\footnotesize $\pm$0.06} \\
            \textbf{letKD-2} & \textbf{76.56 {\footnotesize $\pm$0.22}} & \textbf{75.19 {\footnotesize $\pm$0.13}} & \textbf{73.27 {\footnotesize $\pm$0.16}} & \textbf{73.38 {\footnotesize $\pm$0.14}} & \textbf{74.62 {\footnotesize $\pm$0.20}} & \textbf{77.09 {\footnotesize $\pm$0.18}} \\
    		\bottomrule
    	\end{tabular}%
     }
\end{wraptable}

==> figures/table_CI_homogeneous_Tiny.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\begin{wraptable}[3]{r}[-5pt]{\linewidth}
% \begin{wraptable}[15]{r}[-5pt]{0.5\linewidth}
    % \vspace{-.9\intextsep}
    % \vspace{-10}
	\centering
	\caption{Top-1 acc. averaged over 3 trials on Tiny-ImageNet with 95\% CI for homogeneous distillation. \textbf{Bold}: best in its category.}
	\label{tab:tinyimagenet_CI_homogeneous}
	\resizebox{.8\linewidth}{!}{%
	\begin{tabular}{ccccc}
		\toprule 
		Archs. $\rightarrow$ & \multicolumn{3}{c}{\textbf{Homogeneous}} \\ \cmidrule{2-4}
		Teacher & WRN-40-2 & WRN-40-2 & RN56 \\  
		Student & WRN-16-2 & WRN-40-1 & RN20 \\ \midrule
		\multirow{2}{*}{Methods $\downarrow$} & 61.26 & 61.26 & 58.34 \\
		& 57.17 & 56.25 & 52.66 \\ \midrule
        TDD & 59.22 & 58.42 & 54.45 \\
        QUEST & 59.86 & 59.13 & 54.53 \\
        \midrule
        \textbf{letKD-1} & 61.42 {\footnotesize $\pm$0.36} & 59.75 {\footnotesize $\pm$0.50} & 55.54 {\footnotesize $\pm$0.33}\\
        \textbf{letKD-2} & \textbf{62.21 {\footnotesize $\pm$0.17}} & \textbf{60.59 {\footnotesize $\pm$0.27}} & \textbf{57.35 {\footnotesize $\pm$0.46}} \\
		\bottomrule
	\end{tabular}%
	}
\end{wraptable}


==> figures/table_CI_sub.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{wraptable}[3]{r}[-5pt]{\linewidth}
    \vspace{-.7\intextsep}
    \centering
    \caption{Mean top-1 acc. with 95\% CI over 5 runs.}
    \label{tab:CI}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{ccccccccccc}
        \toprule 
        Dataset $\rightarrow$ & \multicolumn{6}{c}{\textbf{CIFAR-100}} & & \multicolumn{3}{c}{\textbf{Tiny-ImageNet}} \\ \cmidrule{2-7} \cmidrule{9-11}
        Setting $\rightarrow$ & \multicolumn{10}{c}{\textbf{Homogeneous Distillation}} \\ \midrule
        Teacher & WRN-40-2 & WRN-40-2 & RN56 & RN110 & RN110 & RN32x4 & & WRN-40-2 & WRN-40-2 & RN56 
        \\  
        Student & WRN-16-2 & WRN-40-1 & RN20 & RN20  & RN32  & RN8x4 & & WRN-16-2 & WRN-40-1 & RN20 
        \\ \midrule
        TDD & 75.01 & 74.04 & 71.53 & - & - & - & & 59.22 & 58.42 & 54.45 \\
        QUEST & 76.10 & 74.58 & 71.84 & 71.89 & 74.08 & 75.88 & & 59.86 & 59.13 & 54.53\\
        \midrule
        \textbf{letKD-1} & 76.29 {\footnotesize $\pm$0.15} & 75.01 {\footnotesize $\pm$0.09} & 72.44 {\footnotesize $\pm$0.24}  & 72.68 {\footnotesize $\pm$0.31} & 74.40 {\footnotesize $\pm$0.14} & 76.70 {\footnotesize $\pm$0.06} & & 61.42 {\footnotesize $\pm$0.36} & 59.75 {\footnotesize $\pm$0.50} & 55.54 {\footnotesize $\pm$0.33} \\
        \textbf{letKD-2} & \textbf{76.56 {\footnotesize $\pm$0.22}} & \textbf{75.19 {\footnotesize $\pm$0.13}} & \textbf{73.27 {\footnotesize $\pm$0.16}} & \textbf{73.38 {\footnotesize $\pm$0.14}} & \textbf{74.62 {\footnotesize $\pm$0.20}} & \textbf{77.09 {\footnotesize $\pm$0.18}} & & \textbf{62.21 {\footnotesize $\pm$0.17}} & \textbf{60.59 {\footnotesize $\pm$0.27}} & \textbf{57.35 {\footnotesize $\pm$0.46}} \\
        \midrule
        Setting $\rightarrow$ & \multicolumn{10}{c}{\textbf{Heterogeneous Distillation}} \\ \midrule
        
        
        {\begin{tabular}{c}
        Teacher \\
        Student \\ \midrule 
        TDD \\
        QUEST \\ \midrule
        \textbf{letKD-1} \\
        \textbf{letKD-2} \\
        \end{tabular}} & \multicolumn{6}{c}{\begin{tabular}{cccc}
        WRN-40-2 & RN32x4 & RN32x4 & RN50 \\
        SNV1 & SNV1 & SNV2 & MNV2 \\ \midrule
        75.60 & - & - & 68.37 \\
        76.75 & 76.28 & 77.09 & 69.81 \\ \midrule
        76.93 {\footnotesize $\pm$0.16} & 76.65 {\footnotesize $\pm$0.24} & 77.75 {\footnotesize $\pm$0.17} & 69.97 {\footnotesize $\pm$0.18} \\
        \textbf{77.08 {\footnotesize $\pm$0.12}} & \textbf{77.30 {\footnotesize $\pm$0.12}} & \textbf{77.95 {\footnotesize $\pm$0.06}} & \textbf{70.39 {\footnotesize $\pm$0.23}} \\
        \end{tabular}} & & \multicolumn{3}{c}{\begin{tabular}{cc}
        WRN-40-2 & RN50 \\
        SNV1  & MNV2 \\ \midrule
        65.27 & 59.09 \\
        65.23 & 59.81 \\ \midrule
        65.70 {\footnotesize $\pm$0.42} & 60.69 {\footnotesize $\pm$0.17} \\
        \textbf{66.15 {\footnotesize $\pm$0.50}} & \textbf{61.15 {\footnotesize $\pm$0.46}} \\
        \end{tabular}}\\ 
		\bottomrule
        \end{tabular}%
     }
\end{wraptable}

==> figures/table_ImageNet_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\begin{table*}[ht]%[13]{r}[-5pt]{0.6\linewidth}
    %\vspace{-.9\intextsep}
	\centering
	\caption{Top-1 and top-5 accuracies on ImageNet. Setting \textbf{(a)}: Teacher and student models are selected as RN34-RN18. Setting \textbf{(b)}: Teacher and student models are selected as RN50-MNV2. \textbf{Bold}: best in its category.}
	\label{tab:imagenet}
        \resizebox{\textwidth}{!}{
	\begin{tabular}{c|ccccccccc}
		\toprule 
		Setting & & Teacher & Student & KD & AT+KD & DKD & QUEST & \textbf{letKD-1} & \textbf{letKD-2} \\ \midrule   
		\multirow{2}{*}{(a)} & Top-1 & 73.31 & 69.75 & 70.66 & 70.70 & 71.70 & 71.67 & 72.33 & \textbf{72.38} \\
		& Top-5 & 91.42 & 89.07 & 89.88 & 90.00 & 90.41 & 90.67 & 91.06 & \textbf{91.15}\\ \midrule
		\multirow{2}{*}{(b)} & Top-1 & 76.13 & 68.87 & 68.58 & 69.56 & 72.05 & 72.54 & 73.78 & \textbf{73.98}\\
		& Top-5 & 92.86 & 88.76 & 88.98 & 89.33 & 91.05 & 91.13 & 91.81 & \textbf{92.00}\\
		\bottomrule
	\end{tabular}%
        }
\end{table*}


==> figures/table_TinyImageNet.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\begin{table}[H]%[13]{r}[-5pt]{0.6\linewidth}
% \begin{wraptable}[15]{r}[-5pt]{0.5\linewidth}
    % \vspace{-.9\intextsep}
    % \vspace{-10}
	\centering
	\caption{Average top-1 accuracies on Tiny-ImageNet over 3 trials. \textbf{Bold}: best in its category.}
	\label{tab:tinyimagenet}
	\resizebox{.7\linewidth}{!}{%
	\begin{tabular}{ccccccc}
		\toprule 
		Archs. $\rightarrow$ & \multicolumn{3}{c}{\textbf{Homogeneous}} & & \multicolumn{2}{c}{\textbf{Heterogeneous}} \\ \cmidrule{2-4} \cmidrule{6-7}
		Teacher & WRN-40-2 & WRN-40-2 & RN56 & & WRN-40-2 & RN50 \\  
		Student & WRN-16-2 & WRN-40-1 & RN20 & & SNV1  & MNV2 \\ \midrule
		\multirow{2}{*}{Methods $\downarrow$} & 61.26 & 61.26 & 58.34 & & 61.26 & 68.97 \\
		& 57.17 & 56.25 & 52.66 & & 60.52 & 58.35 \\ \midrule
        KD & 59.16 & 57.75 & 53.04 & & 64.80 & 58.68 \\
        FitNet & 57.75 & - & 51.73 & & - & 57.55 \\
        AT & 58.71 & 57.41 & 54.01 & & 63.90 & 50.91\\
        FSP & 57.33 & - & 53.55 & & - & - \\
        SP & 55.69 & 53.74 & 54.03 & & 64.62 & 58.11 \\
        VID & 58.51 & 57.45 & 53.20 & & 63.58 & 57.50 \\
        TDD & 59.22 & 58.42 & 54.45 & & 65.27 & 59.09 \\
        $\underset{\text{+CRD}}{\text{TDD}}$ & 59.53 & 59.20 & 54.85 & & 65.50 & 59.72\\
        QUEST & 59.86 & 59.13 & 54.53 & & 65.23 & 59.81 \\
        \midrule
        \textbf{letKD-1} & 61.42 & 59.75 & 55.54 & & 65.70 & 60.69 \\
        \textbf{letKD-2} & \textbf{62.21} & \textbf{60.59} & \textbf{57.35} & & \textbf{66.15} & \textbf{61.15} \\
		\bottomrule
	\end{tabular}%
	}
\end{table}


==> figures/table_TinyImageNet_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


% \begin{table}[ht]%[13]{r}[-5pt]{0.6\linewidth}
\begin{wraptable}[15]{r}[-5pt]{0.5\linewidth}
    \vspace{-.9\intextsep}
    % \vspace{-10}
	\centering
	\caption{Average top-1 accuracies on Tiny-ImageNet over 3 trials. \textbf{Bold}: best in its category.}
	\label{tab:tinyimagenet}
	\resizebox{\linewidth}{!}{%
	\begin{tabular}{ccccccc}
		\toprule 
		Archs. $\rightarrow$ & \multicolumn{3}{c}{\textbf{Homogeneous}} & & \multicolumn{2}{c}{\textbf{Heterogeneous}} \\ \cmidrule{2-4} \cmidrule{6-7}
		Teacher & WRN-40-2 & WRN-40-2 & RN56 & & WRN-40-2 & RN50 \\  
		Student & WRN-16-2 & WRN-40-1 & RN20 & & SNV1  & MNV2 \\ \midrule
		\multirow{2}{*}{Methods $\downarrow$} & 61.26 & 61.26 & 58.34 & & 61.26 & 68.97 \\
		& 57.17 & 56.25 & 52.66 & & 60.52 & 58.35 \\ \midrule
        KD & 59.16 & 57.75 & 53.04 & & 64.80 & 58.68 \\
        FitNet & 57.75 & - & 51.73 & & - & 57.55 \\
        AT & 58.71 & 57.41 & 54.01 & & 63.90 & 50.91\\
        FSP & 57.33 & - & 53.55 & & - & - \\
        SP & 55.69 & 53.74 & 54.03 & & 64.62 & 58.11 \\
        VID & 58.51 & 57.45 & 53.20 & & 63.58 & 57.50 \\
        TDD & 59.22 & 58.42 & 54.45 & & 65.27 & 59.09 \\
        $\underset{\text{+CRD}}{\text{TDD}}$ & 59.53 & 59.20 & 54.85 & & 65.50 & 59.72\\
        QUEST & 59.86 & 59.13 & 54.53 & & 65.23 & 59.81 \\
        \midrule
        \textbf{letKD-1} & 61.42 & 59.75 & 55.54 & & 65.70 & 60.69 \\
        \textbf{letKD-2} & \textbf{62.21} & \textbf{60.59} & \textbf{57.35} & & \textbf{66.15} & \textbf{61.15} \\
		\bottomrule
	\end{tabular}%
	}
\end{wraptable}


==> figures/table_subclass_value_offline_effect.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


% \begin{table*}[ht]%[13]{r}[-5pt]{0.6\linewidth}
% \begin{table}[H]
%     %\vspace{-.9\intextsep}
% 	\centering
% 	\caption{}
% 	\label{tab:subclass_value_offline}
% 	\resizebox{\linewidth}{!}{%
%     	\begin{tabular}{c|c|c|c|c|c|}
%     		\cline{2-6} 
%     		  & \multirow{2}{*}{Sub + QUEST-\textbf{\emph{R}}} & \multicolumn{2}{c|}{Sub-\textbf{\emph{R}} + QUEST-\textbf{\emph{R}}} & \multirow{2}{*}{Teacher} & \multirow{2}{*}{Student} \\ \cline{3-4}
%              & & \multicolumn{1}{c|}{Before \textbf{\emph{R}}} & \multicolumn{1}{c|}{After \textbf{\emph{R}}} & & \\ \hline
%              \multicolumn{1}{|c|}{GAP} & 52.71 & 51.71 & 56.36 & 47.89 & 51.24 \\ \hline
%              \multicolumn{1}{|c|}{8-sub} & 14.79 & 15.51 & 14.59 & 12.46 & 9.47 \\ \hline
%              \multicolumn{1}{|c|}{1-sub} & 16.95 & 17.80 & 17.06 & 12.13 & 11.17 \\ 
%              \hline        
%     	\end{tabular}%
%     }
% % \end{table*}
% \end{table}

% \begin{table}[H]
%     %\vspace{-.9\intextsep}
% 	\centering
% 	\caption{}
% 	\label{tab:subclass_value_offline}
% 	\resizebox{\linewidth}{!}{%
%     	\begin{tabular}{c|c|c|c|}
%     		\cline{2-4} 
%     		  & \multirow{2}{*}{Sub + QUEST-\textbf{\emph{R}}} & \multicolumn{2}{c|}{Sub-\textbf{\emph{R}} + QUEST-\textbf{\emph{R}}} \\ \cline{3-4}
%              & & \multicolumn{1}{c|}{Before \textbf{\emph{R}}} & \multicolumn{1}{c|}{After \textbf{\emph{R}}} \\ \hline
%              \multicolumn{1}{|c|}{GAP} & 52.71 & 51.71 & 56.36 \\ \hline
%              \multicolumn{1}{|c|}{8-sub} & 14.79 & 15.51 & 14.59 \\ \hline
%              \multicolumn{1}{|c|}{1-sub} & 16.95 & 17.80 & 17.06 \\ 
%              \hline        
%     	\end{tabular}%
%     }
% % \end{table*}
% \end{table}

\begin{wraptable}[9]{r}[-5pt]{0.55\linewidth}
% \vspace{-.8\intextsep}
	\centering
	\caption{Effect of our KD layer on intermediate layer classification performance on CIFAR-100 with RN56-RN20}
	\label{tab:subclass_value_offline}
    	\begin{tabular}{ccc}
    	\toprule
    	\multirow{2}{*}{letKD-2 ($\alpha_{inter}=0$)} & \multicolumn{2}{c}{letKD-2 ($\alpha_{inter}=1$)} \\ \cmidrule{2-3}
        & $x$ & $\hat{x}$ \\ \midrule
        52.71 & 51.71 & 56.36 \\ \bottomrule
    	\end{tabular}%
% \end{table*}
\end{wraptable}

==> figures/table_value_effect.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


% \begin{table*}[ht]%[13]{r}[-5pt]{0.6\linewidth}
%     %\vspace{-.9\intextsep}
% 	\centering
% 	\caption{\textbf{Evaluation on different distillation schemes.} Teacher and student models are selected as ResNet56-ResNet20. All results are the average over 5 trials.}
% 	\label{tab:alldata}
% 	\begin{tabular}{ccccc}
% 		\toprule 
% 		\multicolumn{1}{|c|}{Sub-class} & \multicolumn{1}{c|}{Residual} & \multicolumn{1}{c|}{QUEST} & \multicolumn{1}{c|}{Residual} & \multicolumn{1}{c|}{Top-1 Acc} \\ \hline
% 		\multicolumn{1}{|c|}{\checkmark}          & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{}      & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{}          \\ \hline
        
% 		\bottomrule
% 	\end{tabular}%
% \end{table*}


% \begin{table}[H]
% \centering
% \caption{}
% \label{tab:value_effect}
%     \resizebox{\linewidth}{!}{%
%         \begin{tabular}{ccccc}
%             \hline
%             \multicolumn{1}{|c|}{Sub-class} & \multicolumn{1}{c|}{Residual} & \multicolumn{1}{c|}{QUEST} & \multicolumn{1}{c|}{Residual} & \multicolumn{1}{c|}{Top-1 Acc.} \\ \hline
%             \multicolumn{1}{|c|}{\checkmark} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{70.64} \\ \hline
%             \multicolumn{1}{|c|}{\checkmark} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{70.80} \\ \hline
%             \multicolumn{1}{|c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{71.84} \\ \hline  
%             \multicolumn{1}{|c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{72.44}   \\ \hline  
%             \multicolumn{1}{|c|}{\checkmark} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{71.70}   \\ \hline 
%             \multicolumn{1}{|c|}{\checkmark} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{72.13} \\ \hline 
%             \multicolumn{1}{|c|}{\checkmark} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{72.78} \\ \hline 
%             \multicolumn{1}{|c|}{\checkmark} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{73.27} \\ \hline 
%         \end{tabular}
%     }
% \end{table}


% \begin{table}[H]
\begin{wraptable}[11]{r}[-5pt]{0.4\linewidth}
\vspace{-.7\intextsep}
\centering
\caption{Effect of the included parts in letKD-2}
\label{tab:value_effect}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{ccccc}
            \toprule 
            Inter. & $\alpha_{inter}$ & Penult. & $\alpha_{penult}$ & Top-1 Acc. \\ \midrule
            \checkmark & 0 & - & 0 & 70.64 \\ 
            \checkmark & 1 & - & 0 & 70.80 \\
            - & 0 & \checkmark & 0 & 71.84 \\  
            - & 0 & \checkmark & 1 & 72.44 \\   
            \checkmark & 0 & \checkmark & 0 & 71.70 \\  
            \checkmark & 0 & \checkmark & 1 & 72.13 \\  
            \checkmark & 1 & \checkmark & 0 & 72.78 \\  
            \checkmark & 1 & \checkmark & 1 & 73.27 \\ 
            \bottomrule
        \end{tabular}
    }
% \end{table}
\end{wraptable}

